Evaluation of Neural Architectures Trained with Square Loss vs Cross-Entropy in Classification Tasks

Modern neural architectures for classification tasks are trained using the cross-entropy loss, which is widely believed to be empirically superior to the square loss. In this work we provide evidence indicating that this belief may not be well-founded. We explore several major neural architectures and a range of standard benchmark datasets for NLP, automatic speech recognition (ASR) and computer vision tasks to show that these architectures, with the same hyper-parameter settings as reported in the literature, perform comparably or better when trained with the square loss, even after equalizing computational resources. Indeed, we observe that the square loss produces better results in the dominant majority of NLP and ASR experiments. Cross-entropy appears to have a slight edge on computer vision tasks. We argue that there is little compelling empirical or theoretical evidence indicating a clear-cut advantage to the cross-entropy loss. Indeed, in our experiments, performance on nearly all non-vision tasks can be improved, sometimes significantly, by switching to the square loss. Furthermore, training with square loss appears to be less sensitive to the randomness in initialization. We posit that training using the square loss for classification needs to be a part of best practices of modern deep learning on equal footing with cross-entropy.

==> MSE & CE loss comparison (extend)/math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> MSE & CE loss comparison (extend)/note.tex <==

A few thoughts:

    This paper showed that even with 1 label / example, replacing softmax-xent with sigmoid-xent gave improvements.  Conjecture: Maybe it's softmax vs. not-softmax rather than square vs. xent? Lots of folks piled on that this was important; there was a lot of anti-softmax sentiment.
    Lots of discussion about the connection to discrete choice models.
    David Berthelot mentioned he already contacted you about Brier score.
    This paper came up, also p.5 of this paper. And this one.

Hope this is useful.

Best,

rif

==> MSE & CE loss comparison (extend)/tables/asr_tr_te.tex <==
\begin{table}[!ht]
\centering
\caption{ASR results on training and test set, error rate}
\label{asr_tr_te}
\resizebox{\textwidth}{!}{
\begin{threeparttable}
\begin{tabular}{cccccccc}
\hline
\hline
\multirow{2}{*}{Model}          & \multirow{2}{*}{Task} & \multicolumn{2}{c}{\begin{tabular}[c]{@{}c@{}}train with \\ square loss (\%)\end{tabular}} & \multicolumn{2}{c}{\begin{tabular}[c]{@{}c@{}}train with \\ cross-entropy (\%)\end{tabular} } & \multicolumn{2}{c}{\begin{tabular}[c]{@{}c@{}}square loss w/ same\\ epochs as CE (\%)\end{tabular}} \\ \cline{3-8} 
                                &                      & Train                   & Test                   & Train                    & Test                   & Train                                          & Test                                          \\ \hline
\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}} Attention+CTC \\ \citep{kim2017joint}\end{tabular}} & TIMIT (PER)   &  0.9      & 20.8           &           4.8                                                              & 20.8                                                                &     0.9      &       20.8                                                                                        \\
                               & TIMIT (CER)   &    4.5    & 32.5     &    11.6                                                                  & 33.4           &    4.5                                                                      &         32.5                                                                                      \\
\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}} VGG+BLSTMP \\ \citep{moritz2019triggered} \end{tabular}}    & WSJ (WER)$^*$    &    0.7     & 5.1          &       0.3                                                           & 5.3          &   0.7                                                                         &     5.1                                                                                        \\
                               & WSJ (CER)$^*$    &     0.3   & 2.4                                       &      0.1                               & 2.5              &        0.3                                                                &         2.4                                                                                    \\
\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}} VGG+BLSTM \\ \citep{moritz2019triggered}\end{tabular}}     & Librispeech (WER)$^*$  & 0.8  & 9.8            &      0.4                                                          & 10.6     &                                                                      0.8          &      10.3                                                                                         \\
                               & Librispeech (CER)$^*$ &  0.6   & 9.7          &  0.3                                                                & 10.7          &      0.6                                                                     &    10.2                                                                                           \\ 
\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}} Transformer \\ \citep{watanabe2018espnet}\end{tabular}}     & WSJ (WER)$^*$  & 0.7  & 5.7            & 0.5   & 5.8     &       0.7          &      5.7                                                                                         \\
 & Librispeech (WER)$^*$ &  0.9   & 9.4   &  1.2  & 9.2          &      0.9 &    9.4                                                                                           \\ \hline
\end{tabular}
\begin{tablenotes}[para,flushleft]
\item [*] For WSJ and Librispeech, we take $10\%$ of the training set for the evaluation of the training error rate.
\end{tablenotes}
\end{threeparttable}
}%
\end{table}

% \begin{table}[!ht]
% \centering
% \caption{ASR results of different speech datasets}
% \label{speech_result}
% \begin{threeparttable}
% \begin{tabular}{cccccc}
% \hline
% \hline
% \multirow{2}{*}{Model}         & \multirow{2}{*}{Task} & \multicolumn{2}{c}{Test (\%)}                                                                                        & \multicolumn{2}{c}{Validation (\%)}                                                                                              \\ \cline{3-6} 
%                               &                       & \begin{tabular}[c]{@{}c@{}}train with \\ square loss\end{tabular} & \begin{tabular}[c]{@{}c@{}}train with\\ cross-entropy\end{tabular} & \begin{tabular}[c]{@{}c@{}}train with \\ square loss\end{tabular} & \begin{tabular}[c]{@{}c@{}}train with\\ cross-entropy\end{tabular} \\ \hline
% \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}} Attention+CTC \\ \citep{kim2017joint}\end{tabular}} & TIMIT (PER)    & 20.8                                                        & \textbf{20.7}            & \textbf{18.1}                                               & 18.3                                                        \\
%                               & TIMIT (CER)    & \textbf{32.3}                                                        & 32.7     & \textbf{30.4}                                               & 31.4                                                    \\
% \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}} VGG+BLSTMP \\ \citep{moritz2019triggered} \end{tabular}}    & WSJ (WER)   & \textbf{5.0}                                                         & 5.4    & \textbf{8.5}                                                & 8.8                                                      \\
%                               & WSJ (CER)      & \textbf{2.4}                                                        & 2.6    & \textbf{3.9}                                                & 4.0         \\
% \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}} VGG+BLSTM \\ \citep{moritz2019triggered}\end{tabular}}    & Librispeech (WER) & \textbf{9.7}                                                       & 10.8      & \textbf{9.5}                                              & 10.7    \\
%                               & Librispeech (CER)  & \textbf{9.5}                                                        & 11.0     & \textbf{9.5}                                                & 11.1                                                     \\ \hline
% \end{tabular}
% \begin{tablenotes}[para,flushleft]
% \label{TER}
% \item [*] We are using the ESPnet toolkit \citep{watanabe2018espnet} for implementation.
% \end{tablenotes}
% \end{threeparttable}
% \end{table}


==> MSE & CE loss comparison (extend)/tables/ce_results.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[!ht]
\centering
\caption{Training with the cross-entropy loss, our results and the reported ones}
\label{ce_results}
\resizebox{\textwidth}{!}{
\begin{threeparttable}

\begin{tabular}{cccc}
\hline
\hline
Model                          & Task                       & Our CE result & CE result in the literature \\ \hline
\multirow{6}{*}{BERT$^*$}          & MRPC (acc./F1)             & 85.0/89.6    & 85.29/89.47 \citep{Wolf2019HuggingFacesTS}                \\
                               & SST-2 (acc.)               & 91.5          & 91.97 \citep{Wolf2019HuggingFacesTS}                       \\
                               & QNLI (acc.)                & 90.7          & 87.46 \citep{Wolf2019HuggingFacesTS}                       \\
                               & QQP (acc./F1)              & 90.7/87.4     & 88.40/84.31 \citep{Wolf2019HuggingFacesTS}                 \\
                        & text5 (acc.)                &      80.5     & N/A                       \\
                               & text20 (acc.)              &  85.2    & N/A        \\       \hline
Transformer-XL                &                          &              &     N/A                        \\ 
LSTM+Attention                &                          &              &     N/A                        \\ 

LSTM+CNN                &                          &           &     N/A                        \\ \hline
\multirow{2}{*}{Attention+CTC} & TIMIT (PER)                & 20.7          & 20.5 \citep{watanabe2018espnet}                       \\
                               & TIMIT (CER)                & 32.7          & 33.7 \citep{watanabe2018espnet}                        \\ \hline
\multirow{2}{*}{VGG+BLSTMP}    & WSJ (WER)                  & 5.4           & 5.3 \citep{watanabe2018espnet}                         \\
                               & WSJ (CER)                  & 2.6           & 2.4 \citep{watanabe2018espnet}                         \\ \hline
\multirow{2}{*}{VGG+BLSTM}     & Librispeech (WER)          &     10.8          &    N/A                         \\
                              & Librispeech (CER)          &    11.0           &     N/A                        \\ \hline
\multirow{2}{*}{Transformer}     & WSJ (WER)          &     5.8          &   5.6                         \\
                              & Librispeech (WER)          &    9.2           &     N/A                        \\ \hline
TCNN                           & MNIST (acc.)               &   98.0            &         97.2 \citep{bai2018empirical}                  \\ \hline
Wide-ResNet                    & CIFAR-10 (acc.)            & 96.5          & 96.11 \citep{zagoruyko2016wide}                      \\ \hline
Visual Transformer                    & CIFAR-10 (acc.)            & 99.2          & 99.16 \citep{50650}                      \\ \hline
ResNet-50                      & ImageNet  (acc./Top-5 acc.) & 76.1/93.0     & 76.0/93.0 \citep{tan2019efficientnet}                   \\ \hline
EfficientNet                   & ImageNet (acc./Top-5 acc.) & 77.2/93.4     & 77.3/93.5 \citep{tan2019efficientnet}                   \\ \hline
\end{tabular}

\begin{tablenotes}[para,flushleft]
\item [*] The implementation in \citep{Wolf2019HuggingFacesTS} is using bert-base-uncased model, we are using bert-base-cased, which will result in a little difference. Also, as they didn't give test set results, here for BERT, we give the results of validation set.
\end{tablenotes}
\end{threeparttable}
}
\end{table}

==> MSE & CE loss comparison (extend)/tables/epoch_reg.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[!ht]
\centering
\caption{Training epochs and regularization term}
\label{epoch_reg}
\begin{threeparttable}
\begin{tabular}{ccccc}
\hline
\multirow{2}{*}{Model} & \multirow{2}{*}{Task} & \multicolumn{2}{c}{Epochs training w/} & \multirow{2}{*}{Regularization Term} \\ \cline{3-4}
                       &                       & Square loss         & CE               &                                      \\ \hline
BERT                   & MRPC/SST-2/QNLI/QQP   & 5/3/3/3             & 3/3/3/3          & 0                                    \\
LSTM+Attention         & MRPC/QNLI/QQP         & 20/20/30            & 20/20/30         & 0                                    \\
LSTM+CNN               & MRPC/QNLI/QQP         & 20/20/20            & 20/20/20         & 0                                    \\
Attention+CTC          & TIMIT                 & 20                  & 20               & 0                                    \\
VGG+BLSTMP             & WSJ                   & 15                  & 15               &  a label smoothing based term                                     \\
VGG+BLSTM              & Librispeech           & 30                  & 20               & 0                                    \\
TCN                    & MNIST                 & 20                  & 20               & 0                                    \\
Wide-ResNet            & CIFAR-10              & 200                 & 200              & 0                                    \\
ResNet-50              & ImageNet              & 168885$^*$              & 112590$^*$           &      $ \frac{10^{-4}}{2}\sum_{i=1}^n\bm{w_i}^2$                                \\
EfficientNet           & ImageNet              & 218949$^*$              & 218949$^*$           &    $ \frac{10^{-5}}{2}\sum_{i=1}^n\bm{w_i}^2$                                  \\ \hline
\end{tabular}
\begin{tablenotes}
\item [*] We give the training steps as in the original implementations. 
\end{tablenotes}
\end{threeparttable}
\end{table}

==> MSE & CE loss comparison (extend)/tables/hyper-paras.tex <==
\begin{wraptable}{r}{0.44\linewidth}
\centering
\vspace{-3mm}
\caption{Rescaling parameters}
\label{hyper-paras}
% \resizebox{\linewidth}{!}{%
\begin{tabular}{cccc}
\hline
Dataset         & \#classes & k  & M  \\ \hline
MRPC            & 2         & 1  & 1  \\
SST-2           & 2         & 1  & 1  \\
QNLI            & 2         & 1  & 1  \\
QQP             & 2         & 1  & 1  \\
text-c5  & 5      & 1 & 1 \\
text-c20           & 20        & 1  & 1  \\
text8        & 27        & 1  & 1  \\
enwik8        & 204        & 1  & 1  \\ 
TIMIT (CER)       & 27        & 1  & 1  \\
TIMIT (WER)       & 42        & 1  & 15 \\
WSJ        & 52        & 1  & 15 \\
Librispeech  & 1000      & 15 & 30 \\
MNIST           & 10        & 1  & 1  \\
CIFAR-10        & 10        & 1  & 1  \\
% CIFAR-100        & 100        & 10  & 1  \\
ImageNet        & 1000      & 15 & 30 \\  \hline
\end{tabular}
% }%
\vspace{-7mm}
\end{wraptable}

==> MSE & CE loss comparison (extend)/tables/init-results.tex <==
\begin{table}[!ht]
\centering
\caption{BERT with different initialization for NLP results}
\label{init-bert}
\begin{tabular}{ccccc}
\hline
             & MRPC      & SST-2 & QNLI & QQP       \\ \hline
CE-init1     & 82.1/87.0 & 94.0  & 90.8 & 88.8/70.5 \\
CE-init2     & 83.1/87.6 & 93.9  & 90.6 & 88.9/70.9 \\
CE-init3     & 81.6/86.4 & 93.7  & 90.2 & 89.0/70.8 \\
CE-init4     & 82.6/86.8 & 93.8  & 90.7 & 88.9/70.9 \\
CE-init5     & 80.9/85.6 & 94.2  & 90.6 & 89.0/70.8 
\\ \hline
CE-Ave & 82.1/86.7 & 93.9 & 90.6 & 88.9/70.8
\\ \hline
Square-init1 & 84.0/88.1 & 94.3  & 90.8 & 88.9/70.9 \\
Square-init2 & 84.1/88.6 & 93.8  & 90.8 & 88.9/70.6 \\
Square-init3 & 84.3/88.4 & 94.3  & 90.2 & 88.9/70.4 \\
Square-init4 & 83.0/87.8 & 93.7  & 90.8 & 88.8/70.5 \\
Square-init5 & 83.4/87.5 & 93.6  & 90.5 & 89.0/70.9 \\ \hline
Square-Ave  &  83.8/88.1 & 93.9  & 90.6  & 88.9/70.7
\\ \hline
\end{tabular}
\end{table}

==> MSE & CE loss comparison (extend)/tables/nlp_acc.tex <==
\begin{table}[!ht]
\centering
\vspace{-5mm}
\caption{NLP results, accuracy}
\label{nlp_acc}
\begin{tabular}{cccccc}
\hline
\hline
Model                              & Task           & \begin{tabular}[c]{@{}c@{}}train with \\ square loss (\%)\end{tabular} & \begin{tabular}[c]{@{}c@{}}train with \\ cross-entropy (\%)\end{tabular}  & \begin{tabular}[c]{@{}c@{}} square loss w/ same \\ epochs as CE (\%)\end{tabular} \\ \hline
\multirow{6}{*}{\begin{tabular}[c]{@{}c@{}}fine-tuned BERT \\ \citep{devlin2018bert}\end{tabular}} & MRPC & \bm{$83.8$}   &    $82.1$   & $83.6$\\
                                  & SST-2   & \bm{$94.0$}                  & $93.9$  & $93.9$ \\
                                  & QNLI     & $\bm{90.6}$           & $\bm{90.6}$  & $\bm{90.6}$\\
                                  & QQP &     $\bm{88.9}$        & $\bm{88.9}$   &$88.8$ \\
                                  & text5 &  \bm{$80.6$}&80.5     & \bm{$80.6$}\\
                                  & text20   &  \bm{$85.6$}                 & 85.2 & \bm{$85.6$} \\
                                  \hline

\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Transformer-XL \\ \citep{dai2019transformer}\end{tabular}} & text8 & \bm{$73.2$}   &    $72.8$   & $73.2$\\
                                  & enwik8   & 76.7                 & \bm{$77.5$}  & $76.7$ \\
                                   \hline
\multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}LSTM+Attention  \\ \citep{chen-etal-2017-enhanced}\end{tabular}}              & MRPC& $\textbf{71.7}$    & $70.9$   & $71.5$\\
                                  & QNLI & $\textbf{79.3}$      & $79.0$     &$\textbf{79.3}$ \\
                                  & QQP  & $\textbf{83.4}$      & $83.1$        &     $\textbf{83.4}$ \\ \hline
\multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}LSTM+CNN \\ \citep{he2016pairwise}\end{tabular}}          & MRPC&           $\bm{73.2}$         &       $69.4$  &   $72.5$   \\
                                  & QNLI &             $\bm{76.0}$          &    $\bm{76.0}$ & $\bm{76.0}$ \\
                                  & QQP  &                  $84.3$     &   $\bm{84.4}$ & $84.3$ \\ \hline
\end{tabular}
\vspace{-3mm}
\end{table}

==> MSE & CE loss comparison (extend)/tables/nlp_data.tex <==
\begin{table}[!ht]
\centering
\vspace{-5mm}
\caption{NLP task statistics and descriptions}
\label{nlp_data}
\resizebox{\textwidth}{!}{
\begin{tabular}{cclccccc}
\hline
\hline
Corpus & \multicolumn{2}{c}{$|$Train$|$} & $|$Test$|$ & \#classes                      & Metric  & Domain              &  \\ \cline{1-7}
MRPC \citep{dolan2005automatically}   & \multicolumn{2}{c}{3.7K}    & 1.7K   & 2  & acc./F1 & news                &  \\
SST-2 \citep{socher2013recursive} & \multicolumn{2}{c}{67K}     & 1.8K   & 2 & acc.    & movie reviews       &  \\
QNLI \citep{rajpurkar2016squad}  & \multicolumn{2}{c}{105K}    & 5.4K   & 2     & acc. & Wikipedia           &  \\
QQP \citep{Quora}   & \multicolumn{2}{c}{364K}    & 391K   & 2  & acc./F1 & social QA questions &  \\ 
text-c5  & \multicolumn{2}{c}{2.1K}  &  0.4K & 5  & acc. &   title of conference              &  \\ text-c20  & \multicolumn{2}{c}{28K}   & 12K   & 20  & acc. &    stack overflow            & \\
text8 \citep{multimedia2009large}   & \multicolumn{2}{c}{90M}    & 5M   & 27  & acc. &  English text              &  \\
enwik8 \citep{multimedia2009large}   & \multicolumn{2}{c}{89M}   &  4.9M  & 204  & acc. &            English Wikipedia     &  \\ \cline{1-7}
\end{tabular}
}
\vspace{-3mm}
\end{table}

==> MSE & CE loss comparison (extend)/tables/nlp_f1.tex <==
\begin{table}[!ht]
\centering
\vspace{-6mm}
\caption{NLP results, F1 scores}
\label{nlp_f1}
\begin{tabular}{cccccc}
\hline
\hline
Model                              & Task           & \begin{tabular}[c]{@{}c@{}}train with \\ square loss (\%)\end{tabular} & \begin{tabular}[c]{@{}c@{}}train with \\ cross-entropy (\%)\end{tabular}  & \begin{tabular}[c]{@{}c@{}} square loss w/ same \\ epochs as CE (\%)\end{tabular} \\ \hline
\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}BERT \\ \citep{devlin2018bert}\end{tabular}} & MRPC & $\bm{88.1}$      &    $86.7$   & $88.0$\\
                                   & QQP &    $\bm{70.9}$          & $70.7$   & $70.7$\\ \hline
\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}LSTM+Attention \\ \citep{chen-etal-2017-enhanced}\end{tabular}}              & MRPC& $\textbf{80.9}$        & $80.6$   & $80.7$\\
                                   & QQP  & $\textbf{62.6}$       & $62.3$        &    $\textbf{62.6}$  \\ \hline
\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}LSTM+CNN \\ \citep{he2016pairwise}\end{tabular}}          & MRPC&           $\bm{81.0}$            &       $78.2$   &   $\textbf{81.0}$   \\
                                   & QQP  &                      $60.3$ &    $\bm{60.5}$ & $60.3$\\ \hline
\end{tabular}
\vspace{-3mm}
\end{table}

==> MSE & CE loss comparison (extend)/tables/nlp_para.tex <==
\begin{table}[!ht]
\vspace{-2mm}
\caption{Hyper-parameters for NLP tasks}
\label{nlp_para}
\begin{threeparttable}
\begin{tabular}{|c|c|c|c|c|c|c|c|}
\hline
\multirow{2}{*}{Model}          & \multirow{2}{*}{Task} & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Batch \\ size\end{tabular}} & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}} max\_seq \\ length\end{tabular}} & \multicolumn{2}{c|}{Learning rate w/} & \multicolumn{2}{c|}{Epochs training w/} \\ \cline{5-8} 
                                &        &               &                             &square loss       &CE       &square loss        &CE        \\ \hline
\multirow{6}{*}{BERT}           & MRPC                  & 32        &128                  &        5e-5              & 2e-5        & 5                  & 3         \\ \cline{2-8} 
                                & SST-2                 & 32    &128                      &         2e-5             & 2e-5        &                 3      & 3         \\ \cline{2-8} 
                                & QNLI                  & 32     &128                     &       2e-5               & 2e-5        &      3                 & 3        \\ \cline{2-8} 
                                & QQP                  & 32    &128                       &          2e-5            & 2e-5        &      3                 & 3      
                                
                                \\ \cline{2-8} 
                                & text5                  & 32     &128                     &       2e-5               & 2e-5        &      3                 & 3        \\ \cline{2-8} 
                                & text20                  & 32    &128                       &          2e-5            & 2e-5        &      3                 & 3         \\ \hline
\multirow{2}{*}{Transformer-XL}       & text8                  &        8      &        70       &      2.5e-4                &      2.5e-4       &         $ 400000^\natural$             &    $400000^\natural$            \\ \cline{2-8} 
                                & enwik8     &    8           &     70                     &      2.5e-5                &   2.5e-4          &   $400000 ^\natural$                     &   $400000 ^\natural$            \\ \hline
\multirow{3}{*}{LSTM+Attention} & MRPC                  &           64          &80        &     2e-4                 &       1e-4      &          25             &   20           \\ \cline{2-8} 
                                & QNLI                  &        32      &       $sent\_len^*$        &    1e-4                  &      1e-4       &   20                    &     20         \\ \cline{2-8} 
                                & QQP                &       64      &  120                &    1e-4                 &    1e-4         &   30                    &  30            \\ \hline
\multirow{3}{*}{LSTM+CNN}       & MRPC                  &        64      &80               &      2e-4                &      1e-4       &          20             &    20          \\ \cline{2-7} 
                                & QNLI     &    32           &          $sent\_len^* $                &      8e-5                &   1e-4          &   20                    &   20           \\ \cline{2-8} 
                                & QQP                &     32      &120                     &       1e-3               &     1e-3        &   20                    &  20            \\ \hline
\end{tabular}
\begin{tablenotes}[para,flushleft]
\item [*] The max sequence length equals the max sentence length of the training set.
\item [$\natural$] training steps.
\end{tablenotes}
\end{threeparttable}
\vspace{-4mm}
\end{table}



==> MSE & CE loss comparison (extend)/tables/nlp_train-test.tex <==
\begin{table}[!ht]
\centering
\caption{NLP results on training and test set, accuracy}
\label{nlp_tr-te_acc}
\begin{tabular}{cccccccc}
\hline
\hline
\multirow{2}{*}{Model}          & \multirow{2}{*}{Task} & \multicolumn{2}{c}{\begin{tabular}[c]{@{}c@{}}train with \\ square loss (\%)\end{tabular}} & \multicolumn{2}{c}{\begin{tabular}[c]{@{}c@{}}train with \\ cross-entropy (\%)\end{tabular} } & \multicolumn{2}{c}{\begin{tabular}[c]{@{}c@{}}square loss w/ same\\ epochs as CE (\%)\end{tabular}} \\ \cline{3-8} 
                                &                       & Train                   & Test                   & Train                    & Test                   & Train                                          & Test                                          \\ \hline
\multirow{6}{*}{\begin{tabular}[c]{@{}c@{}}BERT \\ \citep{devlin2018bert}\end{tabular}} & MRPC                  & 99.7                    & 83.8                   & 99.9                     & 82.1                   & 99.6                                           & 83.6                                          \\
                                & SST-2                 & 98.6                    & 94.0                   & 99.2                     & 93.9                   & 98.6                                           & 93.9                                          \\
                                & QNLI                  & 98.0                    & 90.6                   & 97.5                     & 90.6                   & 98.0                                           & 90.6                                          \\
                                & QQP                   & 96.2                    & 88.9                   & 98.0                     & 88.9                   & 96.2                                           & 88.8                                          \\ 
                         & text5                  & 96.7                    & 80.6                   & 96.3                     & 80.5                   & 96.7                                          & 80.6                                          \\
                                & text20                   & 95.6                    & 85.6                   & 94.9                     & 85.2                   & 95.6                                           & 85.6                                          \\         \hline
\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Transformer-XL  \\ \citep{dai2019transformer}\end{tabular}} & text8                  & 90.5                    & 73.2                   & 90.1                     & 72.8                   & 90.5                                           & 73.2                                          \\
                                & enwik8                  & 90.7                    & 76.7                   & 91.8                     & 77.5                   & 90.7                                           & 76.7                                          \\ \hline
\multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}LSTM+Attention  \\ \citep{chen-etal-2017-enhanced}\end{tabular}} & MRPC                  & 94.6                    & 71.7                   & 84.9                     & 70.9                   & 93.2                                           & 71.5                                          \\
                                & QNLI                  & 87.7                    & 79.3                   & 90.8                     & 79.0                   & 87.7                                           & 79.3                                          \\
                                & QQP                   & 93.7                    & 83.4                   & 91.5                     & 83.1                   & 93.7                                           & 83.4                                          \\ \hline
\multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}LSTM+CNN \\ \citep{he2016pairwise}\end{tabular}}       & MRPC                  & 98.3                    & 73.2                   & 92.5                     & 69.4                   & 98.3                                           & 72.5                                          \\
                                & QNLI                  & 92.8                    & 76.0                   & 90.7                     & 76.0                   & 92.8                                           & 76.0                                          \\
                                & QQP                   & 91.3                    & 84.3                   & 95.7                     & 84.4                   & 91.3                                           & 84.3                                          \\ \hline
\end{tabular}
\end{table}

==> MSE & CE loss comparison (extend)/tables/nlp_train-test_f1.tex <==
\begin{table}[!ht]
\centering
\caption{NLP results on training and test set, F1 scores}
\label{nlp_tr-te_f1}
\begin{tabular}{cccccccc}
\hline
\hline
\multirow{2}{*}{Model}          & \multirow{2}{*}{Task} & \multicolumn{2}{c}{\begin{tabular}[c]{@{}c@{}}train with \\ square loss (\%)\end{tabular}} & \multicolumn{2}{c}{\begin{tabular}[c]{@{}c@{}}train with \\ cross-entropy (\%)\end{tabular} } & \multicolumn{2}{c}{\begin{tabular}[c]{@{}c@{}}square loss w/ same\\ epochs as CE (\%)\end{tabular}} \\ \cline{3-8} 
                                &                       & Train                & Test                & Train                    & Test                   & Train                        & Test                       \\ \hline
\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}BERT \\ \citep{devlin2018bert}\end{tabular}}                            & MRPC                  & 99.8                 & 88.1                & 99.9                     & 86.7                   & 99.7                         & 88.0                       \\
                                & QQP                   & 94.5                 & 70.9                & 97.2                     & 70.7                   & 94.5                         & 70.7                       \\ \hline
\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}LSTM+Attention \\ \citep{chen-etal-2017-enhanced}\end{tabular}}  & MRPC                  & 96.1                 & 80.9                & 89.5                     & 80.6                   & 94.7                         & 80.7                       \\
                                & QQP                   & 91.9                 & 62.6                & 89.2                     & 62.3                   & 91.9                         & 62.6                       \\ \hline
\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}LSTM+CNN \\ \citep{he2016pairwise}\end{tabular}}       & MRPC                  & 98.8                 & 81.0                & 94.5                     & 78.2                   & 98.8                         & 81.0                       \\
                                & QQP                   & 88.0                 & 60.3                & 94.2                     & 60.5                   & 88.0                         & 60.3                       \\ \hline
\end{tabular}
\end{table}

==> MSE & CE loss comparison (extend)/tables/nlp_train_acc.tex <==
\begin{table}[!ht]
\centering
\caption{NLP results on training set, accuracy}
\label{nlp_tr_acc}
\begin{tabular}{cccccc}
\hline
\hline
Model                              & Task           & \begin{tabular}[c]{@{}c@{}}train with \\ square loss (\%)\end{tabular} & \begin{tabular}[c]{@{}c@{}}train with \\ cross-entropy (\%)\end{tabular}  & \begin{tabular}[c]{@{}c@{}} square loss w/ same \\ epochs as CE (\%)\end{tabular} \\ \hline
\multirow{4}{*}{\begin{tabular}[c]{@{}c@{}}BERT \\ \cite{devlin2018bert}\end{tabular}} & MRPC & 99.7  &  99.9   & 99.6 \\
                                   & SST-2   &   98.6              & 99.2  & 98.6\  \\
                                   & QNLI     &   98.0       &  97.5 & 98.0\\
                                   & QQP &  96.2           & 98.0  &  96.2  \\ \hline
\multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}LSTM+Attention  \\ \cite{chen-etal-2017-enhanced}\end{tabular}}              & MRPC& 94.6   & 84.9  & 93.2\\
                                   & QNLI &  87.7   &  90.8   &  87.7  \\
                                   & QQP  & 93.7    &91.5& 93.7\\ \hline
\multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}LSTM+CNN \\ \cite{he2016pairwise}\end{tabular}}          & MRPC&         98.3        &  92.5    &98.3     \\
                                   & QNLI &        92.8            &  90.7   &  92.8 \\
                                   & QQP  & 91.3                     & 95.7   &  91.3\\ \hline
\end{tabular}
\end{table}

==> MSE & CE loss comparison (extend)/tables/nlp_train_f1.tex <==
\begin{table}[!ht]
\centering
\caption{NLP results on training set, F1 scores}
\label{nlp_tr_f1}
\begin{tabular}{cccccc}
\hline
\hline
Model                              & Task           & \begin{tabular}[c]{@{}c@{}}train with \\ square loss (\%)\end{tabular} & \begin{tabular}[c]{@{}c@{}}train with \\ cross-entropy (\%)\end{tabular}  & \begin{tabular}[c]{@{}c@{}} square loss w/ same \\ epochs as CE (\%)\end{tabular} \\ \hline
\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}BERT \\ \cite{devlin2018bert}\end{tabular}} & MRPC &  99.8   &  99.9  & 99.7 \\
                                   & QQP &  94.5           & 97.2  & 94.5 \\ \hline
\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}LSTM+Attention \\ \cite{chen-etal-2017-enhanced}\end{tabular}}              & MRPC&   96.1      &  89.5  & 94.7 \\
                                   & QQP  &     91.9   & 89.2       &  91.9   \\ \hline
\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}LSTM+CNN \\ \cite{he2016pairwise}\end{tabular}}          & MRPC&       98.8                &   94.5    &  98.8    \\
                                   & QQP  & 88.0                     & 94.2   & 88.0 \\ \hline
\end{tabular}
\end{table}

==> MSE & CE loss comparison (extend)/tables/nlp_vad_acc.tex <==
\begin{table}[!ht]
\centering
\caption{NLP results on validation set, accuracy}
\label{nlp_vad_acc}
\begin{tabular}{cccccc}
\hline
\hline
Model                              & Task           & \begin{tabular}[c]{@{}c@{}}train with \\ square loss (\%)\end{tabular} & \begin{tabular}[c]{@{}c@{}}train with \\ cross-entropy (\%)\end{tabular}  & \begin{tabular}[c]{@{}c@{}} square loss w/ same \\ epochs as CE (\%)\end{tabular} \\ \hline
\multirow{6}{*}{\begin{tabular}[c]{@{}c@{}}BERT \\ \citep{devlin2018bert}\end{tabular}} & MRPC &  $\bm{85.3}$ &  $85.0$     & $\bm{85.3}$ \\
                                   & SST-2   &  $91.2$                & $\bm{91.5}$  & $91.2$\  \\
                                   & QNLI     &   $\bm{90.8}$         &  $90.7$  & $\bm{90.8}$\\
                                   & QQP &   $\bm{90.8}$          & $90.7$   & $90.6$\\
                         & text5     &   $\bm{80.8}$         &  $80.6$  & $\bm{80.8}$\\
                                   & text20 &   $\bm{85.9}$          & $85.4$   & $\bm{85.9}$\\ \hline   
\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Transformer-XL  \\ \citep{dai2019transformer} \end{tabular}}              & text8&  $\bm{73.4}$  & $72.9$  & $\bm{73.4}$\\
                                   & enwik8 &   $77.0$   &  $\bm{77.8}$   & $77.0$ \\ \hline
\multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}LSTM+Attention  \\ \citep{chen-etal-2017-enhanced}\end{tabular}}              & MRPC&  $\bm{76.5}$  & $74.8$  & $75.3$\\
                                   & QNLI &   $\bm{79.7}$   &  $\bm{79.7}$   & $\bm{79.7}$ \\
                                   & QQP  &   $\bm{86.0}$    &  $85.5$    &   $\bm{86.0}$   \\ \hline
\multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}LSTM+CNN \\ \citep{he2016pairwise}\end{tabular}}          & MRPC&  $\bm{76.0}$                &$73.3$       & $\bm{76.0}$    \\
                                   & QNLI &    $\bm{76.8}$                 &  $\bm{76.8}$   &  $\bm{76.8}$ \\
                                   & QQP  &  $84.0$                    &  $\bm{85.3}$  & $84.0$ \\ \hline
\end{tabular}
\end{table}

==> MSE & CE loss comparison (extend)/tables/nlp_val_f1.tex <==
\begin{table}[!ht]
\centering
\caption{NLP results on validation set, F1 scores}
\label{nlp_val_f1}
\begin{tabular}{cccccc}
\hline
\hline
Model                              & Task           & \begin{tabular}[c]{@{}c@{}}train with \\ square loss (\%)\end{tabular} & \begin{tabular}[c]{@{}c@{}}train with \\ cross-entropy (\%)\end{tabular}  & \begin{tabular}[c]{@{}c@{}} square loss w/ same \\ epochs as CE (\%)\end{tabular} \\ \hline
\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}BERT \\ \citep{devlin2018bert}\end{tabular}} & MRPC & $89.5$     &  $\bm{89.6}$  & $89.5$\\
                                   & QQP &   $\bm{87.5}$          & $87.4$  & $87.4$\\ \hline
\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}LSTM+Attention \\ \citep{chen-etal-2017-enhanced}\end{tabular}}              & MRPC&   $\bm{83.7}$      & 83.3   &  83.5\\
                                   & QQP  &  $\bm{82.1}$      &   $81.7$     &   $\bm{82.1}$  \\ \hline
\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}LSTM+CNN \\ \citep{he2016pairwise}\end{tabular}}          & MRPC&  $\bm{82.6}$                     &  $81.4$      &   $\bm{82.6}$   \\
                                   & QQP  &    $77.4$                  & $\bm{80.2}$   & $77.4$ \\ \hline
\end{tabular}
\end{table}

==> MSE & CE loss comparison (extend)/tables/reg_term.tex <==
\begin{table}[!ht]
\centering
\caption{Regularization term for each task}
\label{reg_term}
\resizebox{\textwidth}{!}{
\begin{threeparttable}
\begin{tabular}{cccccc}
\hline
Model        & Task      & dropout$^*$ & batch norm & Regularization Term \\ \hline

BERT           & \begin{tabular}[c]{@{}c@{}}MRPC/SST-2/QNLI/QQP \\ text5/text20\end{tabular}       &  0.1   & N    & 0                   \\
Transformer-XL    &  text8/enwik8   & 0.1      & N  & 0                   \\
LSTM+Attention & MRPC/QNLI/QQP    &  0.5   & N      & 0                   \\
LSTM+CNN       & MRPC/QNLI/QQP    &   0.0  & N      & 0                   \\
Attention+CTC  & TIMIT     &  0.0   &   N   & 0                   \\
VGG+BLSTMP     & WSJ     &  0.0    &   N    &    label smoothing based                 \\
VGG+BLSTM      & Librispeech &   0.2    &   N   & 0                   \\
Transformer      & WSJ/Librispeech &   0.1    &   N   & 0                   \\
TCN            & MNIST       &   0.05    &  N    & 0                   \\
Wide-ResNet    & CIFAR-10    &   0.0    &  N    & 0                   \\
Visual Transformer    & CIFAR-10    &   0.0    &  N    & 0                   \\
ResNet-50      & ImageNet    &  0.0     &  Y    &   $ \frac{10^{-4}}{2}\sum_{i=1}^n\bm{w_i}^2$                  \\
EfficientNet   & ImageNet    &   0.0    &  Y    &   $ \frac{10^{-5}}{2}\sum_{i=1}^n\bm{w_i}^2$                  \\ \hline
\end{tabular}
\begin{tablenotes}[para,flushleft]
\item[$*$] For dropout, 0.0 means have not apply dropout. 
\end{tablenotes}
\end{threeparttable}
}
\end{table}

==> MSE & CE loss comparison (extend)/tables/reg_yn.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[!ht]
\centering
\caption{With or without regularization}
\label{reg_ys}
\begin{tabular}{cccccc}
\hline
                              & \multirow{2}{*}{Regularization} & \multicolumn{2}{c}{Square loss (Training/Test)} & \multicolumn{2}{c}{CE (Training/Test)} \\
                              &                                 & Top-1                  & Top-5                  & Top-1              & Top-5             \\ \hline
ResNet-50                     & yes                             & 77.7/76.2              & 93.2/93.0              & 80.5/76.1          & 93.4/93.0         \\
                              & no                              & 73.2/73.1              & 91.1/91.1              & 71.1/71.1          & 89.8/89.8         \\
\multirow{2}{*}{EfficientNet} & yes                             & 75.1/74.6              & 93.0/92.7              & 81.4/77.0          & 94.0/93.3         \\
                              & no                              & 65.6/62.1              & 88.1/84.5              & 79.9/74.6          & 93.0/92.0         \\ \hline
\end{tabular}
\end{table}

==> MSE & CE loss comparison (extend)/tables/speech_data.tex <==
\begin{table}[htbp]
\centering
\vspace{-3mm}
\caption{ASR task statistics and descriptions}
\label{speech_data}
\begin{threeparttable}
\begin{tabular}{cccccc}
\hline
\hline
Corpus                       & $|$ Train$|$                               & $|$ Test$|$     & \#classes  & Metric   & Domain                                      \\ \hline
\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}} TIMIT \\ \citep{garofolo1993darpa} \end{tabular}}       & \multirow{2}{*}{1.15M} & \multirow{2}{*}{54K}  & 42    & PER         & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}3.2 hours (training set) \\ telephone English\end{tabular}} \\ 
                             &                        &                       &     27   &            CER                 &                                             \\
\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}} WSJ \\ \citep{paul1992design}\end{tabular}}         & \multirow{2}{*}{28.8M} & \multirow{2}{*}{252K}  & \multirow{2}{*}{$52^*$} & WER          & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}80 hours (training set) \\ read newspapers\end{tabular}}    \\
                             &                        &                        &                       &CER            &                                             \\
\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}} Librispeech \\ \citep{panayotov2015librispeech}\end{tabular}} & \multirow{2}{*}{36M}   & \multirow{2}{*}{1M} & \multirow{2}{*}{$1000^*$}& WER       & \multirow{2}{*}{ \begin{tabular}[c]{@{}c@{}} 100 hours (training set) \\ audio books\end{tabular}}      \\
                             &                        &                        &                        & CER           &                                             \\ \hline
\end{tabular}
\begin{tablenotes}[para,flushleft]
\label{TER}
\item [*] This is the number of classes used for training the acoustic model.
\end{tablenotes}
\end{threeparttable}
\vspace{-2mm}
\end{table}

==> MSE & CE loss comparison (extend)/tables/speech_para.tex <==
\begin{table}[!ht]
\centering
\vspace{-2mm}
\caption{Hyper-parameters for ASR tasks}
\label{speech_para}
\begin{threeparttable}
\begin{tabular}{|c|c|c|c|c|}
\hline
\multirow{2}{*}{Model} & \multirow{2}{*}{Task} & \multirow{2}{*}{Hyper-parameters} & \multicolumn{2}{c|}{Epochs training w/} \\ \cline{4-5} 
                       &                       &                                   & square loss             & CE            \\ \hline
Attention+CTC          & TIMIT                 &      conf/train.yaml$^\natural$                              &        20                 &      20         \\ \hline
VGG+BLSTMP             & WSJ$^*$                   &     conf/tuning/train\_rnn.yaml                              &     15                    &       15        \\ \hline
VGG+BLSTM              & Librispeech           &     conf/tuning/train\_rnn.yaml$^\diamondsuit$                              &           30              &       20        \\ \hline
Transformer              & WSJ           &     conf/tuning/train\_pytorch\_transformer.yaml                              &           100             &       100        \\ \hline
Transformer              & Librispeech           &     conf/tuning/train\_pytorch\_transformer.yaml                              &           120             &       100        \\ \hline
\end{tabular}

\begin{tablenotes}[para,flushleft]
\item [*] For WSJ, we use the language model given by \url{https://drive.google.com/open?id=1Az-4H25uwnEFa4lENc-EKiPaWXaijcJp}.
\item[$\natural$] We set mtlalpha=0.3, batch-size=30. 
\item[$\diamondsuit$] We set elayers=4, as we use 100 hours training data.
\end{tablenotes}
\end{threeparttable}
\vspace{-4mm}
\end{table}

==> MSE & CE loss comparison (extend)/tables/speech_result.tex <==
\begin{table}[!ht]
\centering
\vspace{-3mm}
\caption{ASR results, error rate}
\label{speech_result}
\resizebox{\textwidth}{!}{
\begin{tabular}{ccccc}
\hline
\hline
\multirow{2}{*}{Model}         & \multirow{2}{*}{Task} & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}train with \\ square loss (\%)\end{tabular}} & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}train with\\ cross-entropy (\%)\end{tabular}} & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}square loss w/ same\\epochs as CE (\%)\end{tabular}} \\
                              &                       &                                                                                         &                                                                                          &                                                                                               \\ \hline
\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}} Attention+CTC \\ \citep{kim2017joint}\end{tabular}} & TIMIT (PER)           & \textbf{20.8}                                                                                    & \textbf{20.8}                                                                            &       \textbf{20.8}                                                                                        \\
                              & TIMIT (CER)           & \textbf{32.5}                                                                           & 33.4                                                                                     &         \textbf{32.5}                                                                                      \\
\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}} VGG+BLSTMP \\ \citep{moritz2019triggered} \end{tabular}}    & WSJ (WER)             & \textbf{5.1}                                                                            & 5.3                                                                                      &     \textbf{5.1}                                                                                          \\
                              & WSJ (CER)             & \textbf{2.4}                                                                            & 2.5                                                                                      &         \textbf{2.4}                                                                                      \\
\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}} VGG+BLSTM \\ \citep{moritz2019triggered}\end{tabular}}     & Librispeech (WER)     & \textbf{9.8}                                                                            & 10.6                                                                                     &      10.3                                                                                         \\
                              & Librispeech (CER)     & \textbf{9.7}                                                                            & 10.7                                                                                     &    10.2                                                                                           \\ 
\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}} Transformer \\ \citep{watanabe2018espnet} \end{tabular}}    & WSJ (WER)             & \textbf{5.7}                                                                            & 5.8                                                                                      &     \textbf{5.7}                                                                                          \\
                              & Librispeech (WER)             & 9.4                                                                           & \textbf{9.2}                                                                                      &         9.4                                                                                      \\                              \hline
\end{tabular}
}
\vspace{-2mm}
\end{table}


==> MSE & CE loss comparison (extend)/tables/speech_val_result.tex <==
\begin{table}[!ht]
\centering
\vspace{-2mm}
\caption{ASR results on validation set, error rate}
\label{speech_val_result}
\resizebox{\textwidth}{!}{
\begin{tabular}{ccccc}
\hline
\hline
\multirow{2}{*}{Model}         & \multirow{2}{*}{Task} & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}train with \\ square loss (\%)\end{tabular}} & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}train with\\ cross-entropy (\%)\end{tabular}} & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}square loss w/ same\\epochs as CE (\%)\end{tabular}} \\
                               &                       &                                                                                         &                                                                                          &                                                                                               \\ \hline
\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}} Attention+CTC \\ \citep{kim2017joint}\end{tabular}} & TIMIT (PER)           &        $\bm{18.1}$                                                                             &            $18.3$                                                                &      $\bm{18.1}$                                                                                         \\
                               & TIMIT (CER)           &         $\bm{30.4}$                                                                   & $31.4$                                                                                     &        $\bm{30.4}$                                                                                       \\
\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}} VGG+BLSTMP \\ \citep{moritz2019triggered} \end{tabular}}    & WSJ (WER)             &          $\bm{8.5}$ &     $8.8 $          &        $\bm{8.5}$ \\
   & WSJ (CER)  &   $\bm{3.9} $ & $4.0$ & $\bm{3.9}$ \\
\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}} VGG+BLSTM \\ \citep{moritz2019triggered}\end{tabular}}     & Librispeech (WER)     &          $\bm{9.3}$  &    $10.7$  &          $9.9$  \\
 & Librispeech (CER)     &         $\bm{9.4}$     &  $11.1$    & $10.2$   \\ 

\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}} Transformer \\ \citep{watanabe2018espnet}\end{tabular}}     & WSJ (WER)     &     $\bm{9.1}$   &  $9.3$  &    $\bm{9.1}$    \\
 & Librispeech (WER)     &         $9.7$     &  $\bm{9.1}$    & $9.7$   \\ \hline
\end{tabular}
}

\end{table}

==> MSE & CE loss comparison (extend)/tables/tfr_results.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[!ht]
\centering
\caption{Transformers on different tasks, accuracy}
\label{transformer}
\begin{tabular}{ccccc}
\hline
\hline
Domain                  & Task (\#class)     & Model                                                                         & square loss   & CE            \\ \hline
\multirow{4}{*}{NLP}    & text-c5 (5)        & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}fine-tuned BERT\\ \citep{devlin2018bert}\end{tabular}}    & \textbf{80.6} & 80.5          \\
                        & text-c20 (20)      &                                                                               & \textbf{85.6} & 85.2          \\
                        & text8 (27)         & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Transformer-XL \\ \citep{dai2019transformer}\end{tabular}}                                                  & \textbf{73.2} & 72.8          \\
                        & enwik8 (204)       &                                                                               & 76.7          & \textbf{77.5} \\ \hline
\multirow{2}{*}{Speech} & WSJ (52)           & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Transformer \\ \citep{watanabe2018espnet}\end{tabular}}                                                  & \textbf{94.3} & 94.2          \\
                        & Librispeech (1000) &                                                                               & 90.6          & 90.8          \\ \hline
\multirow{2}{*}{Vision} & CIFAR-10 (10)           & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Visual Transformer \\ \citep{dosovitskiy2020image}\end{tabular}} &        \textbf{99.3}       & 99.2         \\
                        & CIFAR-100 (100)          &                                                                               &     92.1          &  \textbf{92.8}         \\ \hline
\end{tabular}
\end{table}

==> MSE & CE loss comparison (extend)/tables/trans_hyp.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[!ht]
\centering
\caption{Hyper-parameters for Transformer architectures}
\label{t-trans-hyp}
\begin{threeparttable}
\begin{tabular}{|c|c|c|c|c|c|c|c|}
\hline
\multirow{2}{*}{Task} & \multirow{2}{*}{Model}                                                        & \multicolumn{2}{c|}{Batch size} & \multicolumn{2}{c|}{Learning rate w/} & \multicolumn{2}{c|}{Epochs training w/} \\ \cline{3-8} 
                      &                                                                               & square loss        & CE         & square loss        & CE            & square loss        & CE          \\ \hline
text-c5               & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}fine-tuned\\ BERT\end{tabular}}    & 32                 & 32         & 2e-5               & 2e-5          & 3                  & 3           \\ \cline{1-1} \cline{3-8} 
text-c20              &                                                                               & 32                 & 32         & 2e-5               & 2e-5          & 3                  & 3           \\ \hline
text8                 & \multirow{2}{*}{Transformer}                                                  & 8                  & 8          & 2.5e-4             & 2.5e-4        & 40000$^*$              & 40000$^*$         \\ \cline{1-1} \cline{3-8} 
enwik8                &                                                                               & 8                  & 8          & 2.5e-4             & 2.5e-4        & 40000$^*$                & 40000$^*$         \\ \hline
WSJ                   & \multirow{2}{*}{Transformer}                                                  & 32                 & 32         & 10                 & 10            & 100                & 100         \\ \cline{1-1} \cline{3-8} 
Librispeech           &                                                                               & 32                 & 32         & 10                 & 10            & 100                & 120         \\ \hline
CIFAR-10              & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Visual\\ Transformer\end{tabular}} & 256                & 256        & 0.03               & 0.03          & 10000$^*$                & 10000$^*$         \\ \cline{1-1} \cline{3-8} 
CIFAR-100             &                                                                               & 256                & 256        & 0.03               & 0.03          & 10000$^*$                & 10000$^*$         \\ \hline
\end{tabular}
\begin{tablenotes}[para,flushleft]
\item [*] We give the training steps as in the original implementations. 
\end{tablenotes}
\end{threeparttable}

\end{table}

==> MSE & CE loss comparison (extend)/tables/variance.tex <==
\begin{wraptable}{r}{0.44\linewidth}
\centering
\vspace{-8mm}
\caption{Standard deviation of test accuracy/error. Smaller number is bolded.}
\label{variance}
\resizebox{\linewidth}{!}{%
\begin{tabular}{cccc}
\hline
\hline
Model                           & Dataset           & Square loss    & CE             \\ \hline
\multirow{6}{*}{BERT}           &   MRPC                &     \textbf{0.484}            &      0.766          \\
                                &    SST-2               &     0.279            &      \textbf{0.173}          \\
                                &  QNLI                 &  0.241
             &      \textbf{0.205}          \\
                                &  QQP                 & \textbf{0.045}               &  0.063              \\
                                &  text5                 &      \textbf{0.147}         &   0.167             \\
                                &  text20                 &       0.172        & \textbf{0.08}               \\ \hline
\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Transformer-XL\end{tabular}} & text8              & \textbf{0.174}  &     0.204      \\
                                & enwik8              & 0.228 &    \textbf{0.102}      \\
                                \hline

\multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}LSTM\\+Attention\end{tabular}} & MRPC              & \textbf{0.484} & 0.786          \\
                                & QNLI              & \textbf{0.210} & 0.371          \\
                                & QQP               & 0.566           & \textbf{0.352} \\ \hline
\multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}LSTM\\+CNN\end{tabular}}       & MRPC              & \textbf{0.322} & 0.383          \\
                                & QNLI             & \textbf{0.173} & 0.286          \\
                                & QQP               & 0.458          & \textbf{0.161} \\ \hline
\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Attention\\+CTC\end{tabular}}  & TIMIT (PER)       & 0.508          & \textbf{0.249} \\
                                & TIMIT (CER)       & \textbf{0.361} & 0.873          \\ \hline
\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}VGG+\\BLSTMP\end{tabular}}     & WSJ (WER)         & \textbf{0.184} & 0.249          \\
                                & WSJ (CER)         & \textbf{0.077} & 0.118          \\ \hline
\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}VGG+\\BLSTM\end{tabular}}      & Libri (WER) & \textbf{0.126} & 0.257          \\
                                & Libri (CER) & \textbf{0.148} & 0.316            \\
\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}} Transformer\end{tabular}}      & WSJ (WER) &  \textbf{0.206}    &    0.276   \\
                                & Libri (WER) &  \textbf{0.102}    &       0.232       \\                                
                                \hline
TCNN                            & MNIST             & \textbf{0.161} & 0.173          \\ \hline
W-ResNet                     & CIFAR-10          & \textbf{0.184} & 0.481          \\ \hline
Visual Transformer                     & CIFAR-10          &  \textbf{0.063}     &  0.075         \\ \hline
\multirow{2}{*}{ResNet-50}      & I-Net (Top-1)          & \textbf{0.032} & 0.045          \\
                                & I-Net (Top-5)         & 0.126          & \textbf{0.045} \\ \hline
\multirow{2}{*}{EfficientNet}   & I-Net (Top-1)         & 0.138          & \textbf{0.122} \\
                                & I-Net (Top-5)         & \textbf{0.089} & \textbf{0.089} \\ \hline
\end{tabular}
}%
\vspace{-18mm}
\end{wraptable}


==> MSE & CE loss comparison (extend)/tables/vision_acc.tex <==


% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[!ht]
\centering
\vspace{-3mm}
\caption{Vision results, accuracy}
\label{vision_result}
% \begin{threeparttable}
\resizebox{\textwidth}{!}{
\begin{tabular}{ccccc}
\hline
\hline
Model                         & Task                  & \begin{tabular}[c]{@{}c@{}}train with\\ square loss (\%)\end{tabular} & \begin{tabular}[c]{@{}c@{}}train with\\ cross-entropy (\%)\end{tabular} & \begin{tabular}[c]{@{}c@{}}square loss w/ same \\ epochs as CE (\%)\end{tabular} \\ \hline
TCNN \citep{bai2018empirical}                         & MNIST (acc.)          & \textbf{97.7}                                                         & \textbf{97.7}                                                           &        \textbf{97.7}                                                                     \\ 
W-Resnet \citep{zagoruyko2016wide}                 & CIFAR-10 (acc.)       & 95.9                                                                  & \textbf{96.3}                                                           &       95.9                                                                      \\ 
Visual transformer \citep{50650}                 & CIFAR-10 (acc.)       & \textbf{99.3}                                                                  & 99.2                                                           &       \textbf{99.3}                                                                       \\ \cline{1-2}
\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}} ResNet-50 \\ \citep{he2016deep}\end{tabular}}    & ImageNet (acc.)       & \textbf{76.2}                                                         & 76.1                                                                    &        76.0                                                                     \\
                              & ImageNet (Top-5 acc.) & \textbf{93.0}                                                         & \textbf{93.0}                                                           &      92.9                                                                       \\ \cline{1-2}
\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}EfficientNet\\ \citep{tan2019efficientnet}\end{tabular}} & ImageNet (acc.)       & 74.6                                                                 & \textbf{77.0}                                                                    & 74.6                                                                            \\
                              & ImageNet (Top-5 acc.) & 92.7                                                                & \textbf{93.3}                                                                    &     92.7                                                                        \\ \hline
\end{tabular}
}
\vspace{-2mm}
\end{table}


==> MSE & CE loss comparison (extend)/tables/vision_data.tex <==
\begin{table}[htbp]
\centering
\vspace{-5mm}
\caption{Vision task statistics and descriptions}
\label{vision_data}
\resizebox{\textwidth}{!}{
\begin{tabular}{cclccccc}
\hline
\hline
% \cline{1-6}
Corpus    & \multicolumn{2}{c}{$|$Train$|$}     & $|$Test$|$           &\#classes      & Metric                & Domain & \\ \hline
MNIST \citep{lecun1998gradient}& \multicolumn{2}{c}{60K}   & 10K    & 10  & acc.   &  $28 \times 28$        &  \\
CIFAR-10 \citep{krizhevsky2009learning}  & \multicolumn{2}{c}{50K}     & 10K     &10     & acc.       &  $32\times32 $          &  \\
% CIFAR-100 \citep{krizhevsky2009learning}  & \multicolumn{2}{c}{50K}     & 10K     &100     & acc.       &  $32\times32 $          &  \\
\begin{tabular}[c]{@{}c@{}} ImageNet\\ \citep{russakovsky2015imagenet} \end{tabular} & \multicolumn{2}{c}{$\sim$1.28M} & 50K\footnote{We report validation set size, as results are on validation, following the papers for ImageNet tasks.}  & 1000 & \begin{tabular}[c]{@{}c@{}} acc.\\Top-5 acc. \end{tabular}& $224\times224$  &\\ \hline
\end{tabular}
\vspace{-3mm}
}
\end{table}

==> MSE & CE loss comparison (extend)/tables/vision_para.tex <==
\begin{table}[!ht]
\centering
\vspace{-2mm}
\caption{Hyper-parameters for vision tasks}
\label{vision_para}
\begin{threeparttable}
\begin{tabular}{|c|c|c|c|c|}
\hline
\multirow{2}{*}{Model} & \multirow{2}{*}{Task} & \multirow{2}{*}{Hyper-parameters} & \multicolumn{2}{c|}{Epochs training w/} \\ \cline{4-5} 
                       &                       &                                   & square loss           & CE              \\ \hline
TCNN                   & MNIST$^\natural$                 &      the default in \citep{bai2018empirical}                             & 20                    & 20              \\ \hline
Wide-ResNet            & CIFAR-10              &   \begin{tabular}[c]{@{}c@{}}   the default in W-ResNet, \\ except wide-factor=20    \end{tabular}                         & 200                   & 200             \\ \hline
Visual Transformer            & CIFAR-10              &   \begin{tabular}[c]{@{}c@{}}   the default in \citep{50650}    \end{tabular}                         & 200                   & 200             \\ \hline
ResNet-50              & ImageNet              &   \begin{tabular}[c]{@{}c@{}} the default in ResNet, \\ for square loss, learning rate=0.3\end{tabular}                                & 168885$^*$                 & 112590$^*$          \\ \hline
EfficientNet           & ImageNet              & \begin{tabular}[c]{@{}c@{}} the default in EfficientNet-B0 \\ of \citep{tan2019efficientnet}  \end{tabular}                               & 218949$^*$                 & 218949$^*$           \\ \hline
\end{tabular}
\begin{tablenotes}[para,flushleft]
\item[$\natural$] We are doing the permuted MNIST task as in \cite{bai2018empirical}.
\item [*] We give the training steps as in the original implementations. 
\end{tablenotes}
\end{threeparttable}
\vspace{-4mm}
\end{table}

==> MSE & CE loss comparison (extend)/tables/vision_tr_te.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[!ht]
\centering
\caption{Vision results on training and test set, accuracy}
\label{vision_tr_te}
% \begin{threeparttable}
\resizebox{\textwidth}{!}{
\begin{tabular}{cccccccc}
\hline
\hline
\multirow{2}{*}{Model}          & \multirow{2}{*}{Task} & \multicolumn{2}{c}{\begin{tabular}[c]{@{}c@{}}train with \\ square loss (\%)\end{tabular}} & \multicolumn{2}{c}{\begin{tabular}[c]{@{}c@{}}train with \\ cross-entropy (\%)\end{tabular} } & \multicolumn{2}{c}{\begin{tabular}[c]{@{}c@{}}square loss w/ same\\ epochs as CE (\%)\end{tabular}} \\ \cline{3-8} 
                                &                      & Train                   & Test                   & Train                    & Test                   & Train                                          & Test                                          \\ \hline
TCNN \citep{bai2018empirical}                         & MNIST (acc.)    & 98.3     & 97.7                                      &      99.5            & 97.7                                     &            98.3          &        97.7                                                                    \\ 
W-Resnet \citep{zagoruyko2016wide}                 & CIFAR-10 (acc.)     &  100.0    & 95.9                                           &     100.0                  & 96.3                                  &     100.0                    &       95.9                                                                      \\
Visual Transformer \citep{50650}                 & CIFAR-10 (acc.)     &  100.0    & 99.3                                           &     100.0                  & 99.2                                  &     100.0                    &       99.3                                                                      \\
\cline{1-2}
\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}} ResNet-50 \\ \citep{he2016deep}\end{tabular}}    & ImageNet (acc.)    &77.7   & 76.2            &       80.5                                      & 76.1           &  77.7                                                       &        76.0                                                                     \\
                              & ImageNet (Top-5 acc.) &93.2 &93.0                                              &  93.4         & 93.0                                &  93.2                        &      92.9                                                                       \\ \cline{1-2}
\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}EfficientNet\\ \citep{tan2019efficientnet}\end{tabular}} & ImageNet (acc.) &  75.1    & 74.6                                                     &    81.4        & 77.0                                                     &     75.1          & 74.6                                                                            \\
                              & ImageNet (Top-5 acc.)&  93.0    & 92.7     & 94.0                                                          & 93.3                                                                &  93.0   &     92.7                                                                        \\ \hline
\end{tabular}
}
\end{table}


==> note.tex <==

A few thoughts:

    This paper showed that even with 1 label / example, replacing softmax-xent with sigmoid-xent gave improvements.  Conjecture: Maybe it's softmax vs. not-softmax rather than square vs. xent? Lots of folks piled on that this was important; there was a lot of anti-softmax sentiment.
    Lots of discussion about the connection to discrete choice models.
    David Berthelot mentioned he already contacted you about Brier score.
    This paper came up, also p.5 of this paper. And this one.

Hope this is useful.

Best,

rif

==> tables/epoch_reg.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[!ht]
\centering
\caption{Training epochs and regularization term}
\label{epoch_reg}
\begin{threeparttable}
\begin{tabular}{ccccc}
\hline
\multirow{2}{*}{Model} & \multirow{2}{*}{Task} & \multicolumn{2}{c}{Epochs training w/} & \multirow{2}{*}{Regularization Term} \\ \cline{3-4}
                       &                       & Square loss         & CE               &                                      \\ \hline
BERT                   & MRPC/SST-2/QNLI/QQP   & 5/3/3/3             & 3/3/3/3          & 0                                    \\
LSTM+Attention         & MRPC/QNLI/QQP         & 20/20/30            & 20/20/30         & 0                                    \\
LSTM+CNN               & MRPC/QNLI/QQP         & 20/20/20            & 20/20/20         & 0                                    \\
Attention+CTC          & TIMIT                 & 20                  & 20               & 0                                    \\
VGG+BLSTMP             & WSJ                   & 15                  & 15               &  a label smoothing based term                                     \\
VGG+BLSTM              & Librispeech           & 30                  & 20               & 0                                    \\
TCN                    & MNIST                 & 20                  & 20               & 0                                    \\
Wide-ResNet            & CIFAR-10              & 200                 & 200              & 0                                    \\
ResNet-50              & ImageNet              & 168885$^*$              & 112590$^*$           &      $ \frac{10^{-4}}{2}\sum_{i=1}^n\bm{w_i}^2$                                \\
EfficientNet           & ImageNet              & 218949$^*$              & 218949$^*$           &    $ \frac{10^{-5}}{2}\sum_{i=1}^n\bm{w_i}^2$                                  \\ \hline
\end{tabular}
\begin{tablenotes}
\item [*] We give the training steps as in the original implementations. 
\end{tablenotes}
\end{threeparttable}
\end{table}

==> tables/init-results.tex <==
\begin{table}[!ht]
\centering
\caption{BERT with different initialization for NLP results}
\label{init-bert}
\begin{tabular}{ccccc}
\hline
             & MRPC      & SST-2 & QNLI & QQP       \\ \hline
CE-init1     & 82.1/87.0 & 94.0  & 90.8 & 88.8/70.5 \\
CE-init2     & 83.1/87.6 & 93.9  & 90.6 & 88.9/70.9 \\
CE-init3     & 81.6/86.4 & 93.7  & 90.2 & 89.0/70.8 \\
CE-init4     & 82.6/86.8 & 93.8  & 90.7 & 88.9/70.9 \\
CE-init5     & 80.9/85.6 & 94.2  & 90.6 & 89.0/70.8 
\\ \hline
CE-Ave & 82.1/86.7 & 93.9 & 90.6 & 88.9/70.8
\\ \hline
Square-init1 & 84.0/88.1 & 94.3  & 90.8 & 88.9/70.9 \\
Square-init2 & 84.1/88.6 & 93.8  & 90.8 & 88.9/70.6 \\
Square-init3 & 84.3/88.4 & 94.3  & 90.2 & 88.9/70.4 \\
Square-init4 & 83.0/87.8 & 93.7  & 90.8 & 88.8/70.5 \\
Square-init5 & 83.4/87.5 & 93.6  & 90.5 & 89.0/70.9 \\ \hline
Square-Ave  &  83.8/88.1 & 93.9  & 90.6  & 88.9/70.7
\\ \hline
\end{tabular}
\end{table}

==> tables/nlp_train_acc.tex <==
\begin{table}[!ht]
\centering
\caption{NLP results on training set, accuracy}
\label{nlp_tr_acc}
\begin{tabular}{cccccc}
\hline
\hline
Model                              & Task           & \begin{tabular}[c]{@{}c@{}}train with \\ square loss (\%)\end{tabular} & \begin{tabular}[c]{@{}c@{}}train with \\ cross-entropy (\%)\end{tabular}  & \begin{tabular}[c]{@{}c@{}} square loss w/ same \\ epochs as CE (\%)\end{tabular} \\ \hline
\multirow{4}{*}{\begin{tabular}[c]{@{}c@{}}BERT \\ \cite{devlin2018bert}\end{tabular}} & MRPC & 99.7  &  99.9   & 99.6 \\
                                   & SST-2   &   98.6              & 99.2  & 98.6\  \\
                                   & QNLI     &   98.0       &  97.5 & 98.0\\
                                   & QQP &  96.2           & 98.0  &  96.2  \\ \hline
\multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}LSTM+Attention  \\ \cite{chen-etal-2017-enhanced}\end{tabular}}              & MRPC& 94.6   & 84.9  & 93.2\\
                                   & QNLI &  87.7   &  90.8   &  87.7  \\
                                   & QQP  & 93.7    &91.5& 93.7\\ \hline
\multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}LSTM+CNN \\ \cite{he2016pairwise}\end{tabular}}          & MRPC&         98.3        &  92.5    &98.3     \\
                                   & QNLI &        92.8            &  90.7   &  92.8 \\
                                   & QQP  & 91.3                     & 95.7   &  91.3\\ \hline
\end{tabular}
\end{table}

==> tables/nlp_train_f1.tex <==
\begin{table}[!ht]
\centering
\caption{NLP results on training set, F1 scores}
\label{nlp_tr_f1}
\begin{tabular}{cccccc}
\hline
\hline
Model                              & Task           & \begin{tabular}[c]{@{}c@{}}train with \\ square loss (\%)\end{tabular} & \begin{tabular}[c]{@{}c@{}}train with \\ cross-entropy (\%)\end{tabular}  & \begin{tabular}[c]{@{}c@{}} square loss w/ same \\ epochs as CE (\%)\end{tabular} \\ \hline
\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}BERT \\ \cite{devlin2018bert}\end{tabular}} & MRPC &  99.8   &  99.9  & 99.7 \\
                                   & QQP &  94.5           & 97.2  & 94.5 \\ \hline
\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}LSTM+Attention \\ \cite{chen-etal-2017-enhanced}\end{tabular}}              & MRPC&   96.1      &  89.5  & 94.7 \\
                                   & QQP  &     91.9   & 89.2       &  91.9   \\ \hline
\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}LSTM+CNN \\ \cite{he2016pairwise}\end{tabular}}          & MRPC&       98.8                &   94.5    &  98.8    \\
                                   & QQP  & 88.0                     & 94.2   & 88.0 \\ \hline
\end{tabular}
\end{table}

==> tables/reg_yn.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[!ht]
\centering
\caption{With or without regularization}
\label{reg_ys}
\begin{tabular}{cccccc}
\hline
                              & \multirow{2}{*}{Regularization} & \multicolumn{2}{c}{Square loss (Training/Test)} & \multicolumn{2}{c}{CE (Training/Test)} \\
                              &                                 & Top-1                  & Top-5                  & Top-1              & Top-5             \\ \hline
ResNet-50                     & yes                             & 77.7/76.2              & 93.2/93.0              & 80.5/76.1          & 93.4/93.0         \\
                              & no                              & 73.2/73.1              & 91.1/91.1              & 71.1/71.1          & 89.8/89.8         \\
\multirow{2}{*}{EfficientNet} & yes                             & 75.1/74.6              & 93.0/92.7              & 81.4/77.0          & 94.0/93.3         \\
                              & no                              & 65.6/62.1              & 88.1/84.5              & 79.9/74.6          & 93.0/92.0         \\ \hline
\end{tabular}
\end{table}

==> tables/tfr_results.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[!ht]
\centering
\caption{Transformers on different tasks, accuracy}
\label{transformer}
\begin{tabular}{ccccc}
\hline
\hline
Domain                  & Task (\#class)     & Model                                                                         & square loss   & CE            \\ \hline
\multirow{4}{*}{NLP}    & text-c5 (5)        & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}fine-tuned BERT\\ \citep{devlin2018bert}\end{tabular}}    & \textbf{80.6} & 80.5          \\
                        & text-c20 (20)      &                                                                               & \textbf{85.6} & 85.2          \\
                        & text8 (27)         & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Transformer-XL \\ \citep{dai2019transformer}\end{tabular}}                                                  & \textbf{73.2} & 72.8          \\
                        & enwik8 (204)       &                                                                               & 76.7          & \textbf{77.5} \\ \hline
\multirow{2}{*}{Speech} & WSJ (52)           & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Transformer \\ \citep{watanabe2018espnet}\end{tabular}}                                                  & \textbf{94.3} & 94.2          \\
                        & Librispeech (1000) &                                                                               & 90.6          & 90.8          \\ \hline
\multirow{2}{*}{Vision} & CIFAR-10 (10)           & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Visual Transformer \\ \citep{dosovitskiy2020image}\end{tabular}} &        \textbf{99.3}       & 99.2         \\
                        & CIFAR-100 (100)          &                                                                               &     92.1          &  \textbf{92.8}         \\ \hline
\end{tabular}
\end{table}

==> tables/trans_hyp.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[!ht]
\centering
\caption{Hyper-parameters for Transformer architectures}
\label{t-trans-hyp}
\begin{threeparttable}
\begin{tabular}{|c|c|c|c|c|c|c|c|}
\hline
\multirow{2}{*}{Task} & \multirow{2}{*}{Model}                                                        & \multicolumn{2}{c|}{Batch size} & \multicolumn{2}{c|}{Learning rate w/} & \multicolumn{2}{c|}{Epochs training w/} \\ \cline{3-8} 
                      &                                                                               & square loss        & CE         & square loss        & CE            & square loss        & CE          \\ \hline
text-c5               & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}fine-tuned\\ BERT\end{tabular}}    & 32                 & 32         & 2e-5               & 2e-5          & 3                  & 3           \\ \cline{1-1} \cline{3-8} 
text-c20              &                                                                               & 32                 & 32         & 2e-5               & 2e-5          & 3                  & 3           \\ \hline
text8                 & \multirow{2}{*}{Transformer}                                                  & 8                  & 8          & 2.5e-4             & 2.5e-4        & 40000$^*$              & 40000$^*$         \\ \cline{1-1} \cline{3-8} 
enwik8                &                                                                               & 8                  & 8          & 2.5e-4             & 2.5e-4        & 40000$^*$                & 40000$^*$         \\ \hline
WSJ                   & \multirow{2}{*}{Transformer}                                                  & 32                 & 32         & 10                 & 10            & 100                & 100         \\ \cline{1-1} \cline{3-8} 
Librispeech           &                                                                               & 32                 & 32         & 10                 & 10            & 100                & 120         \\ \hline
CIFAR-10              & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Visual\\ Transformer\end{tabular}} & 256                & 256        & 0.03               & 0.03          & 10000$^*$                & 10000$^*$         \\ \cline{1-1} \cline{3-8} 
CIFAR-100             &                                                                               & 256                & 256        & 0.03               & 0.03          & 10000$^*$                & 10000$^*$         \\ \hline
\end{tabular}
\begin{tablenotes}[para,flushleft]
\item [*] We give the training steps as in the original implementations. 
\end{tablenotes}
\end{threeparttable}

\end{table}
